Learning to Generate Novel Scene Compositions from Single Images and Videos

Training GANs in low-data regimes remains a challenge, as overfitting often leads to memorization or training divergence. In this work, we introduce One-Shot GAN that can learn to generate samples from a training set as little as one image or one video. We propose a two-branch discriminator, with content and layout branches designed to judge the internal content separately from the scene layout realism. This allows synthesis of visually plausible, novel compositions of a scene, with varying content and layout, while preserving the context of the original sample. Compared to previous single-image GAN models, One-Shot GAN achieves higher diversity and quality of synthesis. It is also not restricted to the single image setting, successfully learning in the introduced setting of a single video.

==> figures/qual_comparison.tex <==
\begin{figure}[t]
\begin{centering}
\setlength{\tabcolsep}{0.0em}
\renewcommand{\arraystretch}{0}
\par\end{centering}
\begin{centering}
\vspace{-1em}
\hfill{}%
	\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c}
			\centering
		Label map & Ground truth & Pix2pixHD & SPADE & CC-FPSE & OASIS\vspace{0.01cm} \tabularnewline
		
%				\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/label_1} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/image_1} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/spade_1} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/nips19_1} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/our_1} \tabularnewline
		
				
		
		
		
		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/label0022} & {\footnotesize{}}
		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/image0022} & {\footnotesize{}}
		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/pix2pix_0022} & {\footnotesize{}}
		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/spade0022} & {\footnotesize{}}
		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/nips0022} & {\footnotesize{}}
		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/our0022} \tabularnewline
		
		
			\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/label1879} & {\footnotesize{}}
		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/image1879} & {\footnotesize{}}
		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/pix2pix_1879} & {\footnotesize{}}
		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/spade1879} & {\footnotesize{}}
		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/nips1879} & {\footnotesize{}}
		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/our1879} \tabularnewline
		
%	
%			\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/label1534} & {\footnotesize{}}
%		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/image1534} & {\footnotesize{}}
%		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/pix2pix_1534} & {\footnotesize{}}
%		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/spade1534} & {\footnotesize{}}
%		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/nips1534} & {\footnotesize{}}
%		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/our1534} \tabularnewline
		
%		\includegraphics[width=0.195\textwidth, height=0.14\textwidth]{figures/qual_comp/label_4} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.14\textwidth]{figures/qual_comp/image_4} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.14\textwidth]{figures/qual_comp/spade_4} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.14\textwidth]{figures/qual_comp/nips19_4} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.14\textwidth]{figures/qual_comp/our_4} \tabularnewline
%		

		
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/label0196} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/image0196} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/spade0196} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/nips0196} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/our0196} \tabularnewline
		
				
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/label_2} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/image_2} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/spade_2} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/nips19_2} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/our_2} \tabularnewline
%
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/label_3} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/image_3} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/spade_3} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/nips19_3} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/our_3} \tabularnewline
		
%			\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/label1913} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/image1913} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/spade1913} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/nips1913} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/our1913} \tabularnewline


	
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/label1548} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/image1548} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/spade1548} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/nips1548} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/our1548} \tabularnewline
		
	
		
	
		
	
		
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/label0058} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/image0058} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/spade0058} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/nips0058} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/our0058} \tabularnewline
		
	

			\end{tabular}
\hfill{}
\par\end{centering}
\vspace{-0.5em}
\caption{\label{fig:qual_comp} Qualitative comparison of OASIS with other methods on ADE20K. Trained with only adversarial supervision, our model generates images with better perceptual quality and structure.}
\vspace{-1em}
\end{figure}




%\begin{figure}[t]
%\begin{centering}
%\setlength{\tabcolsep}{0.0em}
%\renewcommand{\arraystretch}{0}
%\par\end{centering}
%\begin{centering}
%\vspace{-1em}
%\hfill{}%
%	\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}}
%			\centering
%		Label map & Real image & SPADE \cite{park2019semantic} & CC-FPSE \cite{liu2019learning} & Our model\vspace{0.05cm} \tabularnewline
%
%
%
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/label0022} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/image0022} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/spade0022} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/nips0022} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/our0022} \tabularnewline
%
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/label0058} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/image0058} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/spade0058} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/nips0058} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/our0058} \tabularnewline
%
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/label0196} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/image0196} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/spade0196} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/nips0196} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/our0196} \tabularnewline
%
%
%			\end{tabular}
%\hfill{}
%\par\end{centering}
%\caption{\label{fig:qual_comp} Qualitative comparison with other methods. Trained without the perceptual loss, our model generates images with better textures, perceptual quality and the color distribution closer to real images. }
%\vspace{-0.5em}
%\end{figure}
%
%
%
%
%
%\begin{figure}[t]
%\begin{centering}
%\setlength{\tabcolsep}{0.0em}
%\renewcommand{\arraystretch}{0}
%\par\end{centering}
%\begin{centering}
%\vspace{-1em}
%\hfill{}%
%	\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}}
%			\centering
%		Label map & Real image & SPADE \cite{park2019semantic} & CC-FPSE \cite{liu2019learning} & Our model\vspace{0.05cm} \tabularnewline
%
%
%
%
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/label1534} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/image1534} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/spade1534} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/nips1534} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/our1534} \tabularnewline
%
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/label1548} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/image1548} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/spade1548} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/nips1548} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/our1548} \tabularnewline
%
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/label1879} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/image1879} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/spade1879} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/nips1879} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/our1879} \tabularnewline
%
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/label1913} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/image1913} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/spade1913} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/nips1913} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/our1913} \tabularnewline
%
%			\end{tabular}
%\hfill{}
%\par\end{centering}
%\caption{\label{fig:qual_comp} Qualitative comparison with other methods. Trained without the perceptual loss, our model generates images with better textures, perceptual quality and the color distribution closer to real images. }
%\vspace{-0.5em}
%\end{figure}
%
%
%


==> figures/qual_results_2images.tex <==
\begin{figure}[h!]
\begin{centering}
\setlength{\tabcolsep}{0.1em}
\renewcommand{\arraystretch}{0}
\par\end{centering}
\begin{centering}
\vspace{-1em}
\hfill{}%
\begin{tabular}{c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c}


\includegraphics[width=0.25\linewidth]{figures/funny_cat} & {\footnotesize{}}
\includegraphics[width=0.25\linewidth]{figures/funny_cat} & {\footnotesize{}}
\includegraphics[width=0.25\linewidth]{figures/funny_cat} & {\footnotesize{}}
\includegraphics[width=0.25\linewidth]{figures/funny_cat}\tabularnewline

\includegraphics[width=0.25\linewidth]{figures/funny_cat} & {\footnotesize{}}
\includegraphics[width=0.25\linewidth]{figures/funny_cat} & {\footnotesize{}}
\includegraphics[width=0.25\linewidth]{figures/funny_cat} & {\footnotesize{}}
\includegraphics[width=0.25\linewidth]{figures/funny_cat}\tabularnewline


\end{tabular}\hfill{}
\par\end{centering}
\vspace{-0.5em}
\caption{\label{fig:qual_2image} Some images from 2 image training
 }
\vspace{0em}
\end{figure}

==> figures/singan_failures.tex <==
\begin{figure}[h!]
	\begin{centering}
		\setlength{\tabcolsep}{0.0em}
		\renewcommand{\arraystretch}{0}
		\par\end{centering}
	\begin{centering}
		\vspace{-1em}
		%\hfill{}%
		\begin{tabular}{@{}c@{\hskip 0.01in}c@{\hskip 0.01in}c@{}}
		 &\multicolumn{2}{c}{\hspace{-0.1in} \small SinGAN~\cite{Shaham2019SinGANLA}, lowest resolution of 20px}  
			\tabularnewline	
	 \multirow{-2}{*}{\begin{tabular}{c}  Training image \\ 	\includegraphics[width=0.3\linewidth, height=0.07\textheight]{figures/singan_failures/colusseum}\end{tabular}  } & 
			\includegraphics[width=0.3\linewidth, height=0.07\textheight]{figures/singan_failures/col5} & 
		%	\includegraphics[width=0.3\linewidth]{figures/singan_failures/col7} & 
			\includegraphics[width=0.3\linewidth, height=0.07\textheight]{figures/singan_failures/col6} 	\tabularnewline
			& \multicolumn{2}{c}{ \hspace{-0.1in}  \small SinGAN~\cite{Shaham2019SinGANLA}, lowest resolution of 35px} \tabularnewline
			
			& \includegraphics[width=0.3\linewidth, height=0.07\textheight]{figures/singan_failures/col2} & 
			\includegraphics[width=0.3\linewidth, height=0.07\textheight]{figures/singan_failures/col1}
		% & 	\includegraphics[width=0.3\linewidth]{figures/singan_failures/col3}
			
			\tabularnewline
			
			
		\end{tabular}\hfill{}
		\par\end{centering}
	\vspace{-0.5em}
	\caption{\label{fig:singan_failures} Limitation of the multi-stage training of single image patch-GAN methods. 
		As the finer generation stages cannot correct the layout decision made by the coarser scale generators, without a careful tuning of the lowest resolution size the model falls into producing images of very low diversity or generating incoherent layouts.		
		%	As the middle and latest stages cannot correct the layout decision of the first scale generators, without a careful balancing the model falls into producing images of very low diversity or generating incoherent layouts.
	}
	\vspace{-1em}
\end{figure}



%\begin{figure*}[h!]
%	\begin{centering}
%		\setlength{\tabcolsep}{0.0em}
%		\renewcommand{\arraystretch}{0}
%		\par\end{centering}
%	\begin{centering}
%		\vspace{-1em}
%		%\hfill{}%
%		\begin{tabular}{c@{\hskip 0.05in}|@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}|c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}}
%			{Training image} &\multicolumn{3}{c|}{SinGAN~\cite{Shaham2019SinGANLA}, with a lowest resolution of 20px}  & \multicolumn{3}{c}{SinGAN~\cite{Shaham2019SinGANLA}, with a lowest resolution of 35px}
%			\tabularnewline	
%			\includegraphics[width=0.13\linewidth]{figures/singan_failures/colusseum} & 
%			\includegraphics[width=0.13\linewidth]{figures/singan_failures/col5} & 
%			\includegraphics[width=0.13\linewidth]{figures/singan_failures/col6} & 
%			\includegraphics[width=0.13\linewidth]{figures/singan_failures/col7} & 
%			\includegraphics[width=0.13\linewidth]{figures/singan_failures/col1} & 
%			\includegraphics[width=0.13\linewidth]{figures/singan_failures/col2} & 
%			\includegraphics[width=0.13\linewidth]{figures/singan_failures/col3}
%			
%			\tabularnewline
%
%			
%		\end{tabular}\hfill{}
%		\par\end{centering}
%	\vspace{-0.5em}
%	\caption{\label{fig:singan_failures} Limitation of the multi-stage training of single image patch-GAN methods. 
%		As the finer generation stages cannot correct the layout decision made by of the coarser scale generators, without a careful tuning of the lowest resolution size the model falls into producing images of very low diversity or generating incoherent layouts.		
%	%	As the middle and latest stages cannot correct the layout decision of the first scale generators, without a careful balancing the model falls into producing images of very low diversity or generating incoherent layouts.
%	}
%	\vspace{0em}
%\end{figure*}

==> tables/comparison_single_image.tex <==
\begin{table}[t]
\vspace{-1em}
	\setlength{\tabcolsep}{0.15em}
	\renewcommand{\arraystretch}{0.95}
	\centering
	
	\begin{tabular}{c|cc|c|c|c}
		\multirow{2}{*}{\normalsize{} Method } &  \multicolumn{2}{c|}{\small{} SIFID \cite{Shaham2019SinGANLA}} & \multirow{2}{*}{\small{} LPIPS$\uparrow$ } & \multirow{2}{*}{\small{} MS-SSIM~$\downarrow$} & {\small{} Pixel~$\uparrow$ }  \tabularnewline
		& \footnotesize{best}~$\downarrow$ & \footnotesize{mean}~$\downarrow$ & & & {\small{} Diversity } \tabularnewline
		
		\hline 	 \hline 	
		
		{\small{} SinGAN \cite{Shaham2019SinGANLA} } & \small{0.09}  & \small{0.15}  &  \small{0.22} & \small{0.75} & \small{0.52}  \tabularnewline

		
		{\small{} ConSinGAN \cite{Hinz2020ImprovedTF} } & \small{0.06}  & \small{0.08}  &    \small{0.24} & \small{0.73} & \small{0.50}  \tabularnewline
		
		{\small{} FastGAN \cite{anonymous2021towards} } & \small{0.11}  & \small{0.14} & \small{0.15} & \small{0.81} & \small{0.48}  \tabularnewline		
		
		{\small{} One-Shot GAN } & \textbf{\small{0.05}}  & \textbf{\small{0.06}} & \textbf{\small{0.28}} & \textbf{\small{0.67}} & \textbf{\small{0.57}}  
		
	\vspace{-0.5em}
		\end{tabular}
		\caption{Comparison with other methods on Places dataset in the Single Image setting.}
	\label{table:comp_single_image} %
	\vspace{-0.5em}
\end{table}


==> tables/comparison_single_image_fid.tex <==
\begin{table}[t]
	\vspace{-1em}
	\setlength{\tabcolsep}{0.7em}
	\renewcommand{\arraystretch}{0.95}
	\centering
	
	\begin{tabular}{c|cccc}
		\multirow{2}{*}{\normalsize{} Method } &  \multicolumn{4}{c}{\normalsize{} SIFID ~$\downarrow$}  \tabularnewline
		& \footnotesize{$\frac{H\times W}{4}$\cite{Shaham2019SinGANLA}} & \footnotesize{$\frac{H\times W}{8}$} & \footnotesize{$\frac{H\times W}{16}$} & \footnotesize{$1\times 1$} \tabularnewline
		
		\hline 	 \hline 	
		
		{\small{} SinGAN \cite{Shaham2019SinGANLA} } & \small{0.15}  & \small{2.55}  &  \small{19.3} & \small{1370}  \tabularnewline

		
		{\small{} ConSinGAN \cite{Hinz2020ImprovedTF} } & \small{0.08}  & \small{1.75}  &    \small{18.9} & \small{1220}  \tabularnewline
		
		{\small{} FastGAN \cite{anonymous2021towards} } & \small{0.14}  & \small{2.83} & \small{15.9} & \small{1020}  \tabularnewline		
		
		{\small{} One-Shot GAN } & \textbf{\small{0.06}}  & \textbf{\small{1.09}} & \textbf{\small{14.4}} & \textbf{\small{880}}  

		\end{tabular}
		\vspace{-0.5em}
		\caption{Comparison with other methods in the Single Image setting using SIFID at different InceptionV3 layers.}
	\label{table:comp_single_image_fid} %
		\vspace{-1em}
\end{table}


==> tables/comparison_single_video.tex <==
\begin{table}[t]

	\vspace{-1em}


	\setlength{\tabcolsep}{0.18em}
	\renewcommand{\arraystretch}{0.95}
	\centering
	
	\begin{tabular}{c|cc|c|c|c}
		\multirow{2}{*}{\normalsize{} Method } &  \multicolumn{2}{c|}{\small{} SIFID~$\downarrow$} & \multirow{2}{*}{\small{} LPIPS~$\uparrow$ } & \multirow{2}{*}{\small{} MS-SSIM~$\downarrow$} & \small{} Dist.~   \tabularnewline
		& \footnotesize{$\frac{H\times W}{4}$} & \footnotesize{$\frac{H\times W}{16}$} & & & to train \tabularnewline
		
		\hline 	\hline 	
		
		{\small{} SinGAN \cite{Shaham2019SinGANLA} } & \color{darkred} \small{2.47}  & \color{darkred} \small{96.35}   &  \small{0.32}  & \small{0.65} &    \small{0.51}  \tabularnewline

		
		{\small{} ConSinGAN \cite{Hinz2020ImprovedTF} } & \color{darkred} \small{2.74} & \color{darkred} \small{74.50}  &    \small{0.34}  & \small{0.62}  &   \small{0.53} \tabularnewline
		
		{\small{} FastGAN \cite{anonymous2021towards} }  & \small{0.79} & \small{9.24}  & \textbf{\small{0.43}} & \small{0.55} &  \color{darkred} \small{0.13}  \tabularnewline
		
		{\small{} One-Shot GAN }  & \textbf{\small{0.55}} & \textbf{\small{5.14}} & \textbf{\small{0.43}} & \textbf{\small{0.54}}  &  \small{0.34}
		\end{tabular}
		\vspace{-0.5em}
			\caption{Comparison in the Single Video setting.}
	\label{table:comp_single_video} %
	\vspace{-1em}
\end{table}


% original table below

%\begin{table}[t]
%	
%	\vspace{-1em}
%	
%	
%	\setlength{\tabcolsep}{0.4em}
%	\renewcommand{\arraystretch}{0.95}
%	\centering
%	
%	\begin{tabular}{c|cc|c|c}
%		\multirow{2}{*}{\normalsize{} Method } &  \multicolumn{2}{c|}{\small{} SIFID~$\downarrow$} & \multirow{2}{*}{\small{} LPIPS~$\uparrow$ } & \multirow{2}{*}{\small{} MS-SSIM~$\downarrow$}   \tabularnewline
%		& \footnotesize{$\frac{H\times W}{4}$} & \footnotesize{$\frac{H\times W}{16}$} & & \tabularnewline
		
%		\hline 	\hline 	
		
%		{\small{} SinGAN \cite{Shaham2019SinGANLA} } & \small{11.10}  & \small{58.72}   &  \small{0.41} & \small{0.59}  \tabularnewline
		
		
%		{\small{} ConSinGAN \cite{Hinz2020ImprovedTF} } & \small{14.30} & \small{72.61}  &    \small{0.39} & \small{0.62}   \tabularnewline
		
%		{\small{} FastGAN \cite{anonymous2021towards} }  & \small{0.71} & \small{3.44}  & \textbf{\small{0.44}} & \textbf{\small{0.53}}   \tabularnewline		
		
%		{\small{} One-Shot GAN }  & \textbf{\small{0.59}} & \textbf{\small{3.29}}  & \small{0.43} & \small{0.54} 
%	\end{tabular}
%	\vspace{-0.5em}
%	\caption{Comparison in the Single Video setting.}
%	\label{table:comp_single_video} %
%	\vspace{-1em}
%\end{table}




==> tables/diversity_ablations.tex <==
\begin{table}[t]
	\vspace{-0.5em}
	\setlength{\tabcolsep}{0.1em}
	\renewcommand{\arraystretch}{0.95}
	\centering
	
	\begin{tabular}{c|c|c|c|c}
		\multirow{2}{*}{\small{Regularization} } & \multirow{2}{*}{\normalsize{} SIFID~$\downarrow$} & \multirow{2}{*}{\small{} LPIPS~$\uparrow$ } & \multirow{2}{*}{\small{} MS-SSIM~$\downarrow$} & {\small{} Pixel ~$\uparrow$}  \tabularnewline
        & & & & \small{} Diversity \tabularnewline
		
		\hline 	\hline 	
		
		{\normalsize None} &  \textbf{\small{0.045}}  &  \small{0.02} & \small{0.99} & \small{0.25}  \tabularnewline

		{\normalsize{} zCR \cite{zhao2020improved} } & \small{0.050}   &  \small{0.02} & \small{0.98} & \small{0.26}  \tabularnewline
		
		{\normalsize{} DS\cite{Yang2019DiversitySensitiveCG}   } & \small{0.048}  &  \small{0.08} & \small{0.88} & {\small{0.33}} \tabularnewline	
	

		%{\normalsize{} DS\cite{Yang2019DiversitySensitiveCG} ($G$ feat.)  } & \small{0.07}  &  \small{0.23} & \small{0.71} & {\small{0.53}} \tabularnewline	
		
			{\normalsize{} DR (im. space)   } & \small{0.066}  &  \small{0.13} & \small{0.84} & {\small{0.45}} \tabularnewline			
		
		{\normalsize{} DR   } & \small{0.063}  &  \small{0.24} & \small{0.72} & {\small{0.53}} \tabularnewline
				
		{\normalsize{} DR + FA   } & \small{0.064}  &  \textbf{\small{0.28}} & \textbf{\small{0.67}} & \textbf{\small{0.57}} 

		\end{tabular}
		\vspace{-0.5em}
		\caption{Ablation on diversity regularization techniques. }
	\label{table:ablation_diversity} %
		\vspace{-1em}
\end{table}


==> tables/diversity_ablations_davis.tex <==
\begin{table}[t]
	\vspace{-0.5em}
	\setlength{\tabcolsep}{0.1em}
	\renewcommand{\arraystretch}{0.95}
	\centering
	
	\begin{tabular}{c|c|c|c|c}
		\multirow{2}{*}{\small{Regularization} } & \multirow{2}{*}{\normalsize{} SIFID~$\downarrow$} & \multirow{2}{*}{\small{} LPIPS~$\uparrow$ } & \multirow{2}{*}{\small{} MS-SSIM~$\downarrow$} & {\small{} Pixel ~$\uparrow$}  \tabularnewline
        & & & & \small{} Diversity \tabularnewline
		
		\hline 	\hline 	
		
		{\normalsize None} &  \textbf{\small{0.05}}  &  \small{0.04} & \small{0.95} & \small{0.33}  \tabularnewline

		{\normalsize{} zCR \cite{Zhao2020ImprovedCR} } & \small{0.05}   &  \small{0.06} & \small{0.93} & \small{0.37}  \tabularnewline
		
		{\normalsize{} DS\cite{Yang2019DiversitySensitiveCG}   } & \small{0.06}  &  \small{0.14} & \small{0.84} & {\small{0.45}} \tabularnewline	
	

		%{\normalsize{} DS\cite{Yang2019DiversitySensitiveCG} ($G$ feat.)  } & \small{0.07}  &  \small{0.23} & \small{0.71} & {\small{0.53}} \tabularnewline	
		
			{\normalsize{} DR (im. space)   } & \small{0.07}  &  \small{0.21} & \small{0.72} & {\small{0.52}} \tabularnewline			
		
		{\normalsize{} DR   } & \small{0.08}  &  \textbf{\small{0.33}} & \textbf{\small{0.63}} & \textbf{{\small{0.66}}} \tabularnewline
				
		%{\normalsize{} DR + FA   } & \small{0.08}  &  \textbf{\small{0.33}} & \textbf{\small{0.63}} & \textbf{\small{0.66}} 

		\end{tabular}
		\vspace{-0.5em}
		\caption{Comparison of diversity regularizations in the Single Image setting on DAVIS-YFCC100M.}
	\label{table:ablation_diversity} %
		\vspace{-1em}
\end{table}


==> tables/main_ablations.tex <==
\begin{table}[t]

\vspace{-1em}
	\setlength{\tabcolsep}{0.2em}
	\renewcommand{\arraystretch}{0.95}
	\centering
	
	\begin{tabular}{c|cc|c|c|c}
		\multirow{2}{*}{\small{} Method } & \multicolumn{2}{c|}{\small{} SIFID~$\downarrow$}  & \multirow{2}{*}{\small{} LPIPS~$\uparrow$ } & \multirow{2}{*}{\small{} MS-SSIM~$\downarrow$} & {\small{} Pixel~$\uparrow$ }  \tabularnewline
		& \footnotesize{}  \footnotesize{$\frac{H\times W}{4}$} & \footnotesize{}  \footnotesize{$\frac{H\times W}{16}$} & & & \small{} Diversity   \tabularnewline
		
		\hline 	\hline 	
		
		{\small{} Baseline  } & \textbf{\small{0.04}} & \textbf{\small{6.9}}  &  \color{darkred}\small{0.07} & \color{darkred} \small{0.91} & \color{darkred} \small{0.31}  \tabularnewline
		
		{\small{} Layout br.   } & \small{0.16}   & \small{18.9}  & \textbf{ \small{0.33}} & \textbf{\small{0.63}} & \textbf{\small{0.58}}  \tabularnewline
		
		{\small{} Content br.   } & \small{0.08} & \small{17.5}  &  \small{0.28} & \small{0.68} & \small{0.56}  \tabularnewline
		
		{\small{} Full model   } & \small{0.06} & \small{14.4} &  \small{0.28} & \small{0.67} & \small{0.57}  \tabularnewline
	
		\end{tabular}
	\vspace{-0.5em}
	\caption{Ablation on the proposed discriminator structure on Places dataset in the Single Image setting. Indicators of collapsed diversity or poor quality are marked in red. 
	% when other methods passed 100.
}
\vspace{-0.5em}
\label{table:main_ablation} %

\end{table}


==> tables/table_with_ablations.tex <==
\begin{table*}[t]

\vspace{-1em}
	\setlength{\tabcolsep}{0.2em}
	\renewcommand{\arraystretch}{0.95}
	\centering
	
	\begin{tabular}{c|cc|c|c|c|c||cc|c|c|c}
		& \multicolumn{6}{c||}{Single Image}  & \multicolumn{5}{c}{Single Video}  
		\tabularnewline
		\multirow{2}{*}{\small{} Method } & \multicolumn{2}{c|}{\small{} SIFID~$\downarrow$}  & \multirow{2}{*}{\small{} LPIPS~$\uparrow$ } & \multirow{2}{*}{\small{} MS-SSIM~$\downarrow$} & {\small{} Pixel~$\uparrow$ } & {\small{} Dist.} &  \multicolumn{2}{c|}{\small{} SIFID~$\downarrow$} & \multirow{2}{*}{\small{} LPIPS~$\uparrow$ } & \multirow{2}{*}{\small{} MS-SSIM~$\downarrow$} & \small{} Dist.~ \tabularnewline
		& \footnotesize{}  \footnotesize{$\frac{H\times W}{4}$} & \footnotesize{}  \footnotesize{$\frac{H\times W}{16}$} & & & \small{} Diversity & {\small{} to train} &\footnotesize{$\frac{H\times W}{4}$} & \footnotesize{$\frac{H\times W}{16}$} & & & to train  \tabularnewline
		
		\hline 	\hline 	
		{\small{} Full model   } & \small{0.08} & \small{16.30} &  \small{0.33} & \small{0.63} & \small{0.66} & \small{0.37} &  \small{0.55} & \small{} 5.14 & \textbf{\small{0.43}} & \textbf{\small{0.54}}  & \small{0.34} 
		 \tabularnewline \hline
		{\small{} No Layout br.   } & \color{darkred} \small{0.14}   & \color{darkred} \small{20.29}  & \textbf{\small{0.35}} & \textbf{\small{0.60}} & \textbf{\small{0.67}} & \small{0.40}  & \color{darkred} \small{} 0.71 & \color{darkred} \small{11.70}   & \small{0.42}  & \textbf{\small{0.54}}  & \small{0.38}   \tabularnewline
		
		{\small{} No Content br.   } & \small{0.08} & \color{darkred}\small{23.25}  &  \small{0.34} & \small{0.62} & \small{0.64} & \small{0.36} & \color{darkred} \small{0.73}  & \color{darkred} \small{10.43}   & \small{0.41}  & \small{0.55}  & \small{0.33}   \tabularnewline
		
		{\small{} No $\mathcal{L}_{D_{low-level}}$ } & \small{0.08} & \small{15.92}  &  \small{0.27} & \small{0.70} & \small{0.56} & \small{0.29} & \small{0.58}  & \small{5.32}  & \small{0.40}  & \small{0.56}  & \small{0.31}   \tabularnewline
		
		{\small{} No DR } & \small{0.05} & \small{11.99}  &  \color{darkred} \small{0.04} & \color{darkred} \small{0.95} & \color{darkred} \small{0.33} &  \small{0.06} & \small{0.40}  & \small{9.81}  & \color{darkred} \small{0.30}   & \color{darkred} \small{0.68}   &  \small{0.32}    \tabularnewline 
		
		{\small{} No FA } & \small{0.08} & \small{14.81}  &  \small{0.27} &  \small{0.68} &  \small{0.58} &  \small{0.33} & \small{0.51}  & \small{4.85} & \small{0.41}   & \small{0.56} &  \small{0.32}   \tabularnewline 
		\hline
		{\small{} Baseline  } & \textbf{\textbf{\small{0.03}}} & \textbf{\textbf{\small{7.73}}}  &  \color{darkred}\small{0.13} & \color{darkred} \small{0.84} & \color{darkred} \small{0.43} & \small{0.12} & \small{0.42}  & \small{3.73}  & \small{} \color{darkred} 0.37 & \color{darkred} \small{0.59}   & \small{0.18}  
 \tabularnewline
	
		\end{tabular}
	\vspace{-0.5em}
	\caption{Ablation study on proposed modifications on DAVIS-YFCC100M in the Single Image and Single Video settings. Indicators of collapsed diversity (low LPIPS, Pixel Divesity, high MS-SSIM) or poor quality (high SIFID) are marked in red. 
	% when other methods passed 100.
}
\vspace{-0.5em}
\label{table:main_ablation} %

\end{table*}


==> tex/method.tex <==
\section{One-Shot GAN}
\label{sec:method}
\input{figures/model_overview}

%model motivation, overview of the model 

In this section, we present our One-Shot GAN model, which in comparison to previous methods~\cite{Shaham2019SinGANLA,Hinz2020ImprovedTF,anonymous2021towards}, can work in different one-shot regimes (single image and single video) and is designed not only to learn the internal patch-based distribution, but also to capture the  high-level content of the image and global layout coherency. The key ingredients of One-Shot GAN is the novel design of the two-branch discriminator (Sec.~\ref{sec:method_discriminator}) and the introduced diversity regularization for one-shot image synthesis (Sec.~\ref{sec:method_DR}).

\subsection{Content-Layout Discriminator} \label{sec:method_discriminator}

One of the challenges of training the GAN model in the one-shot setting regime is the problem of overfitting to the original sample. In many cases the model can simply memorize the original training image, and its augmentations (if used during the training). To avoid the memorization effect, \cite{Shaham2019SinGANLA,Hinz2020ImprovedTF} proposed to learn the internal patch-based distribution by using a hierarchy of patch-GANs \cite{isola2017image,Li2016PrecomputedRT} at different scales. Because the employed patch-GANs have small receptive fields and limited capacity, it prevents them from memorizing the overall image. However, as a downside those models can only synthesize images of low-level diversity tuned to the chosen minimal size and number of scales.  If the image contains a more complex scene, they quite often generate images with incoherent global layouts (see Fig.~\ref{} \anna{need to show the example here to proof the point}), and thus do not generalize well to other settings, such as learning from a single video (see Table~\ref{table:comp_single_video}).  

We therefore introduce an alternative solution to overcome the memorization effect but still to produce images of high-level diversity. In particular, we propose a two-branch discriminator, disentangling its decision about the content and layout realism of the image into separate branches. Note that the branching of the discriminator happens after intermediate feature layers; this is done in order to learn the relevant representations for building the content and layout branches.  
The discriminator judging the internal content distribution irrespective from the scene layout realism, and vice versa, enables the generator to synthesize images with varying content and global layouts.
In order to also preserve the good low-level details of the generated images, such as textures, we additionally ask the discriminator to make the real/fake decision based on the feature representations extracted at the lower intermediate layers (before branching). 
The loss of the new discriminator $D$ is then computed by taking the decisions from the content branch $D_{content}$, the layout branch $D_{layout}$ and from the low-level features of the discriminator $D_{low-level}$:
\begin{align}
& \mathcal{L}_{D}  = \mathcal{L}_{D_{low-level}} + \mathcal{L}_{D_{content}} + \mathcal{L}_{D_{layout}}, \label{eq:loss_d}
\end{align} 
where $\mathcal{L}_{D_{*}} = -\mathbb{E}_x[\log D_{*}(x)]- \mathbb{E}_z[\log (1-D_{*}(G(z)))]$.
The architecture of the content-layout discriminator is depicted in Figure \ref{fig:model_over}, and its branches are described below.

\paragraph{Content branch}
The decision of the content branch of the discriminator should be based upon the internal content of the image - the fidelity of "objects" composing the image, independent of their spatial location in the image layout.
%\textit{content} -- the presence of elements/parts composing the object, and \textit{location} -- the spatial placement and arrangement of these parts.
Let the dimension of the input feature map $F_{input}$ of the content branch be $H\times W\times C$, where $H$, $W$, $C$ are the height, width and channels of the feature map. Note that the spatial resolution $H\times W$ captures spatial information and channels $C$ encode feature representations. Upon removing the spatial information from the channels, the network is induced to respond to the content features encoded in different channels irrespective of their spatial location. Hence, we propose to aggregate the spatial information $H\times W$ across the channels $C$ in order to remove the layout information and allow the network to make its decisions based on the feature representation encoded in spatially aggregated channels $F_{content}$ with size $1\times\ 1\times C$. For the spatial aggregation we use average pooling ...

\anna{mention here feature augmentations specific to the content branch to encourage content diversity}
\anna{formalize discriminator content loss, mention loss for intermediate layers}

\paragraph{Layout branch}

\anna{mention here feature augmentations specific to the layout branch to encourage layout diversity}
\anna{formalize discriminator layout loss, mention loss for intermediate layers}

%\paragraph{Feature and data augmentations}
%data augmentations
%feature augmentations for different branches 


full loss for new 2-branch D

\subsection{Diversity Regularization} \label{sec:method_DR}

To improve the variability of the generated image samples, we propose to add diversity regularization (DR) loss term $\mathcal{L}_{DR}$ to the One-Shot GAN objective.
Prior work of \cite{Yang2019DiversitySensitiveCG,Zhao2020ImprovedCR} also proposed to use diversity regularization for GAN training, but mainly to avoid mode collapse and assuming the availability of a large set of training samples. The regularization of \cite{Yang2019DiversitySensitiveCG} aimed to encourage the generator to produce different outputs depending on the input latent code, in such way that the generated samples with closer latent codes should look more similar to each other, and vice versa.
In contrast, our diversity regularization is tuned for one-shot image synthesis. Assuming that in the one-shot mode we are operating in one semantic domain, the generator should produce images that are in-domain but more or less equally different from each other and substantially diverse form the original training sample. In the one-shot image synthesis setting, the perceptual distance of the generated images should not be dependent on the distance between their latent codes.
Thus, we propose to encourage the generator to produce perceptually different image samples independent of their distance in the latent space. Mathematically, the new diversity regularization is expressed as follows:
\begin{align}
\mathcal{L}_{DR} (G) = \mathbb{E}_{z_1,z_2}\big[\frac{1}{L}\sum_{l=1}^{L}\|G^{l}(z_1)-G^{l}(z_2)\|)\big], \label{loss_DR}
\end{align}
where $\|\cdot\|$ denotes the norm, $G^{l}(z)$ indicates a feature extracted from $l$th layer of the generator $G$ given input $z$, and $z_1, z_2$ are randomly sampled latent codes in the batch, i.e. $z_1,z_2 \sim N(0,1)$.
By regularizing generator to maximize Eq.~\ref{loss_DR}, we force the generator to produce diverse outputs for different latent codes $z$.
Note that, in contrast to \cite{Yang2019DiversitySensitiveCG,Zhao2020ImprovedCR}, we compute the distance between samples in the feature space of the generator. Computing the sample distance in the feature space enables more meaningful diversity of the generated images. Different layers of the generator capture different semantics of the image, inducing both high-level and low-level diversity in samples.
Computing the sample distance directly from the generator outputs (in the pixel space), as in \cite{Yang2019DiversitySensitiveCG,Zhao2020ImprovedCR}, i.e. $\|G(z_1)-G(z_2)\|$, in our experiments leads to limited diversity and also worse quality of the generated samples.

An overall One-Shot GAN objective can be written as:
\begin{align}
\min_{G} \max_{D} \hspace{0.5em} \mathcal{L}_{GAN} (G,D) - \lambda \mathcal{L}_{DR} (G), \label{loss_full}
\end{align}
where $\lambda$ controls the strength of the diversity regularization and $\mathcal{L}_{GAN}$ is the adversarial loss.
%The adversarial loss is expressed as: 
%\begin{align*}
%\mathcal{L}_{GAN} (G,D) = \mathbb{E}_x[\log D(x)] + \mathbb{E}_z[\log (1-D(x,G(z)))],
%%$\label{eq:loss_gan}
%\end{align*}
%where the two-branch discriminator $D$ aims to distinguish between real $x$ and generated $G(z)$ images based on their content and layout realism.
The proposed diversity regularization is simple, can be easily integrated into different GAN objectives, and highly-effective for the one-shot image synthesis task, where previous diversity regularizations~\cite{Yang2019DiversitySensitiveCG,Zhao2020ImprovedCR} fail (see Sec.~\ref{sec:exp_sin_image} and Table~\ref{table:ablation_diversity}).

\subsection{Implementation and Training}

architecture details, training details

==> tex/related_work.tex <==
\section{Related Work}
\label{sec:related_work}
%\paragraph{One-Shot Generative Models}
\paragraph{Single Image Generative Models}
Several works investigated learning generative models from a single image.
\cite{Ulyanov2018DeepIP,Shocher2018ZeroShotSU} showed that, when trained on a single image, a deep convolutional network can learn a useful representation which captures the internal distribution of that image. These learned representations can be employed to synthesize textures from a sample texture image \cite{Jetchev2016TextureSW,Bergmann2017LearningTM,Ulyanov2016TextureNF,Zhou2018NonstationaryTS,Li2016PrecomputedRT,Ulyanov2017ImprovedTN}, to "blindly" super-resolve \cite{Shocher2018ZeroShotSU,BellKligler2019BlindSK,Lugmayr2020SRFlowLT} or inpaint the image~\cite{Ulyanov2018DeepIP}. 
Recently, single image GAN models \cite{Shocher2019InGANCA,Shaham2019SinGANLA} have been proposed, revealing the power of image priors learned from a single natural image for synthesis and manipulation tasks. InGAN \cite{Shocher2019InGANCA} introduced an internal GAN based model conditioned on a single natural image, which can remap the input to any size or shape while preserving its internal distribution. SinGAN \cite{Shaham2019SinGANLA} employed an unconditional GAN to produce images of arbitrary size from noise and used a multi-stage training scheme to learn the multi-scale patch distribution of an image.
ConSinGAN \cite{Hinz2020ImprovedTF} extended SinGAN by improving the rescaling for multi-stage training and training several stages concurrently, which allowed to reduce the size of the model and make the training more efficient. 
To explore the semantic meaning of patches inside a single image, \cite{Li2020SemanticIA} used a conditional single image GAN with the segmentation map as dense conditional input.
%\cite{Vinker2020TrainingES} proposed a non-adversarial approach for single image generative modeling by exploiting a VAE.
%Inspired by single-image generative models, \cite{Gur2020HierarchicalPV} introduced the patch VAE-GAN method for unconditional video generation from a single video sample.

%In contrast to 
Contrary to single image GANs of \cite{Shocher2019InGANCA,Shaham2019SinGANLA,Hinz2020ImprovedTF}, our model is not only aimed to learn the internal patch-based distribution of the image, but is designed to capture the coherent global layouts and high-level content of the image. This enables synthesis of higher diversity without losing quality and fidelity to the original image.
Our model is more universal: it can effectively operate in different low-data regimes, such as training from a single image or a single video, 
%and a few samples training, 
and thus can be applied in many real-world scenarios. % more useful for real-world applications.   

 %\anna{todo: add differences to our model, 1. multiple low-data regime settings, single-image and single-video 2. different technical solution, our model not only tuned to capture patch distribution but also layout, thus more diverse images with better quality}

%
%


\paragraph{Few-Shot Generative Models}
Few-shot image generation seeks to generate more data of a given domain, with only few available training samples.
Many of existing few-shot image generation methods resorted to using large image sets of seen classes to train a conditional GAN model, which is then used to generate new images for an unseen class based on a few examples \cite{Hong2020DeltaGANTD, Antoniou2017DataAG, Hong2020F2GANFG}. \cite{Antoniou2017DataAG} injected random noise into the generator conditioned on an image to produce a slightly different sample from the same class. \cite{Hong2020MatchingganMF,Hong2020F2GANFG} proposed to fuse the information from multiple conditional images of the same class.
Other works focused on improving the sample efficiency of GANs by few-shot adaptation \cite{Mo2020FreezeDA, Wang2020MineGANEK, Robb2020FewShotAO, Wang2018TransferringGG,Noguchi2019ImageGF}. These methods usually start from GAN models pre-trained on large datasets and adapt them on few samples in the target domain by fine-tuning all weights of the generator and discriminator \cite{Wang2018TransferringGG}, freezing lower layers of the discriminator \cite{Mo2020FreezeDA}, changing only batch statistics \cite{Noguchi2019ImageGF}, restricting the space of trainable parameters \cite{Robb2020FewShotAO}, or transferring the knowledge via a miner network \cite{Wang2020MineGANEK}.
Contrary to our work, the above methods heavily rely on \emph{external} knowledge from a pre-trained GAN, 
%to achieve good results in the target domain 
and their performance highly depends on the semantic consistency between the target domain and the pre-trained model.
In practice, there is no guarantee that a compatible pre-training dataset is available, and pre-training on semantically incompatible samples might lead to even worse performance \cite{Zhao2020DifferentiableAF}.


Another line of work focused on improving the stability of GANs when trained with limited data. To prevent the overfitting of the discriminator, \cite{Karras2020TrainingGA,Zhao2020ImageAF,Zhao2020DifferentiableAF} explored different data augmentation schemes for both real and generated images. Similarly to them, we also employ augmentation for training, exploring both image and feature augmentations to improve diversity of the generated samples while operating in one-shot mode.  
Most recently, FastGAN \cite{anonymous2021towards} has proposed to train from scratch an unconditional GAN model for few-shot image synthesis. %with low computational cost. 
To avoid the risk of overfitting and mode-collapse, they enabled the fast learning of the generator through a skip-layer channel-wise excitation module and used a self-supervised discriminator %trained as a feature-encoder 
to continuously provide useful signals to the generator. However, 
to achieve good results FastGAN requires sufficient number of training samples ($\sim 100$), while our model needs as little as one image sample (see Sec.~\ref{sec:exp_sin_image} and Table~\ref{table:comp_single_image_fid}). 


%here models in a few-shot setting, both for conditional/unconditional gans
%
%few-shot image synthesis:
%Towards Faster and Stabilized GAN Training for High-fidelity Few-shot Image Synthesis
%\cite{anonymous2021towards}

%techniques that stabilize the GAN training with an improved synthesis quality, given sub-hundred high-fidelity images and a limited computing resource.

%F2GAN: Fusing-and-Filling GAN for Few-shot Image Generation \cite{Hong2020F2GANFG}
%DeltaGAN: Towards Diverse Few-shot Image Generation with Sample-Specific Delta \cite{Hong2020DeltaGANTD}
%
%
%
%few-shot image translation:
%Few-Shot Unsupervised Image-to-Image Translation \cite{Liu2019FewShotUI}
%TuiGAN: Learning Versatile Image-to-Image Translation with Two Unpaired Images \cite{Lin2020TuiGANLV}


%GANs trained with limited training data:
%Training Generative Adversarial Networks with Limited Data \cite{Karras2020TrainingGA}
%Image Augmentations for GAN Training \cite{Zhao2020ImageAF}

